Towards Practical Meshlet Compression

We propose a codec specifically designed for meshlet compression, optimized for rapid data-parallel GPU decompression within a mesh shader. Our compression strategy orders triangles in optimal generalized triangle strips (GTSs), which we generate by formulating the creation as a mixed integer linear program (MILP). Our method achieves index buffer compression rates of 16:1 compared to the vertex pipeline and crack-free vertex attribute quantization based on user preference. The 15.5 million triangles of our teaser image decompress and render in 0.59 ms on an AMD Radeon RX 7900 XTX.

==> secs/meshshadingpipeline.tex <==
\subsection{Geometry Pipelines}\label{Sec:MeshShadingPipeline}
\begin{figure}
    \sf
    \centering
    \def\svgwidth{\columnwidth}    
    \fontsize{4.5pt}{5.5pt}\selectfont%
    \input{figs/GraphicsPipeline_Small_tex.pdf_tex}
    \caption{The graphics pipeline. The graphics pipeline consists of the geometry, raster, and pixel stage.
    There are two ways to program the geometry stage: the \emph{vertex pipeline} (top) and the \emph{mesh-shading pipeline} (bottom). 
    Note that the raster and the pixel stage is the same for both pipelines.
    Each stage has programmable shader and fixed function units.    
    }
    \label{fig:GraphicsPipeline}
\end{figure}
\noindent%
Since our technique makes use of mesh-shading, we briefly discuss its predecessor, which we refer to as the \emph{vertex pipeline}.
Mesh-shading highly relates to compute shaders, so before detailing out mesh-shaders, we recap the most important concepts of compute shaders.

Most of the information here is due to the Direct3D12 specification~\cite{DirectXSpecs} and we stick to its definitions and limits.
% Author Information:
%-------------------
% Use these terms
%----------------
% Geometry Stage
% Pixel Stage
% Raster Stage
% Vertex Pipeline
% Mesh Shading Pipeline (NOT Mesh SHADER Pipeline)
% Vertex Shader
% Hull Shader
% Domain Shader
% Geometry Shader
% Pixel Shader
% Mesh Shader
% Amplification Shader (NOT Acceleration Shader)
% Thread
% Thread Group
% Group-Shared Memory
% Wave
% Device Memory
% Compute Unit
The \ac{GPU} rasterization pipeline of Fig.~\ref{fig:GraphicsPipeline} consists of a \emph{geometry stage} and a \emph{pixel stage} bridged by the \emph{raster stage}.
The geometry stage outputs vector information, like triangles, points, or lines, to the raster stage.
The raster stage discretizes this information into fragments.
Finally, the pixel stage transforms fragments to the output image pixels.

There are two ways to program the geometry stage: the \emph{vertex pipeline} and the \emph{mesh-shading pipeline}. 
The programming model of the vertex pipeline of Fig.~\ref{fig:GraphicsPipeline} (left) takes on a geometry-centric view.
In contrast, the programming model of mesh-shading pipeline of Fig.~\ref{fig:GraphicsPipeline} (right) is almost identical to the one used by compute shaders.
Therefore, it allows the programmer to exploit \ac{GPU} capabilities that cannot be exposed by the domain-specific vertex pipeline programming model.
But both pipelines feed vector information to the raster stage in two different ways.

\subsubsection{Vertex Pipeline}\label{Sec:VertexPipeline}
Before the introduction of the mesh-shading pipeline in 2018~\cite{Kubisch18Introduction}, the only way to program the geometry stage is through the vertex pipeline using vertex, geometry, hull, and domain shaders as shown in the left of Fig.~\ref{fig:GraphicsPipeline}.
These shader programs are expressed with respect to individual vertices, samples, and primitives.
Likewise, domain shaders operate on samples in a 1D or 2D domain, hull shaders on control vertices of higher-order patches, and geometry shaders on either points, lines, or triangles.
A vertex shader instance obtains the attributes of a single vertex, transforms it, and outputs the transformed vertex attributes. 
Each vertex shader instance is independent from all others which allows for a high degree of parallelism.
Depending on vertex reuse in the index buffer and on the caching of the transformed vertex shader output, a single vertex might be processed multiple times.

\subsubsection{Compute Shader}
As an alternative way to program the geometry pipeline, mesh-shading relates to the model of \emph{compute shaders}.
There, a program contains the instructions a single \emph{thread} executes.
% 1024 work-items: 
% - D3D12: 
%    https://learn.microsoft.com/en-us/windows/win32/direct3d12/constants
%   D3D12_CS_THREAD_GROUP_MAX_THREADS_PER_GROUP
% - Vulkan:
%    https://vulkan.gpuinfo.org/displaydevicelimit.php?name=maxComputeWorkGroupInvocations&platform=all
Up to 1024 threads form a \emph{thread group}. 
Each thread group is executed on one of the \ac{GPU}'s hardware \emph{compute units}.
A compute unit executes subsets of threads within the same thread group -- called \emph{wave} -- in parallel.
Further, a fast \emph{group-shared memory} on each compute unit and \emph{barriers} enable communication and synchronization between threads of the same thread group.
A \ac{CPU} program typically dispatches multiple thread groups and the \ac{GPU} usually possesses multiple compute units to execute several thread groups in parallel.

\subsubsection{Mesh-Shading Pipeline}
% Explain mesh shaders
The core of the mesh-shading pipeline, shown in the right of Fig.~\ref{fig:GraphicsPipeline}, is its mandatory programmable \emph{mesh-shader}.
A mesh-shader is similar to a compute shader: 
its code specifies the instruction of a thread within a thread group and the programmer dispatches multiple thread groups.
The key difference to a compute shader is that each mesh-shader thread group outputs a small mesh -- called \emph{meshlet} -- to the raster stage.
A meshlet consists of a local vertex-buffer with per-vertex attributes and an index-buffer whose elements point into the local vertex-buffer.
% Output: 
% D3D12:    Primitives:  256
%           Vertices:   256
% Vulkan:   Primitives: 256  (AMD), 256-512 (Nvidia) 1024 (Intel)               
%           https://vulkan.gpuinfo.org/displayextensionproperty.php?extensionname=VK_EXT_mesh_shader&extensionproperty=maxMeshOutputPrimitives&platform=all
%           https://vulkan.gpuinfo.org/displayextensionproperty.php?extensionname=VK_NV_mesh_shader&extensionproperty=maxMeshOutputPrimitives&platform=all
%           Vertices:   256  (AMD), 256-512 (Nvidia) 1024 (Intel)
A meshlet consists of up to 256 vertices and 256 primitives.

% Difference to compute shaders
%
% Work-Items
% D3D12: https://microsoft.github.io/DirectX-Specs/d3d/MeshShader.html 
% - 128
% Vulkan: http://vulkan.gpuinfo.org/displayextensionproperty.php?extensionname=VK_EXT_mesh_shader&extensionproperty=maxMeshWorkGroupInvocations&platform=all
% 128 (Nvidia), 256 (AMD), 1024 (Intel)
% 
A mesh-shader thread group may use group-shared memory and barriers, but it is limited to 128 threads.
Note that a compute shader could conceptually produce output equivalent to that of a mesh shader.
However, a compute shader must write its output to global \ac{GPU} \emph{device memory} first.
Then, a vertex pipeline needs to read that output again only to hand it over to the raster stage.
With the mesh-shading pipeline, we get the advantage of directly passing meshlets to the raster stage without the extra read and write to device memory.

% Amplification Shaders
The \emph{amplification shader} stage is optional and runs before the mesh-shader stage.
It is similar to a compute shader, but it has the ability to dispatch mesh-shader thread groups.
For example, an amplification shader may dispatch a varying number of mesh-shader thread groups depending on an object's level-of-detail.
An amplification shader may even dispense mesh-shader thread-group execution if its corresponding meshlet is not visible.

% Difference to Vertex Pipeline
% Input Assembly
Note that the mesh-shading pipeline has no \emph{input assembler}.
In the vertex pipeline, the input assembler extracts each vertex and its attributes from global index and vertex buffers.
The vertex-shader instance then obtains this information.
Except for specifying the input layout, this process is transparent to the programmer.
With the mesh-shading pipeline, however, the programmer must explicitly provide code to read all the information from device memory to compute meshlets for the raster stage.
Also note that the vertex pipeline uses a single-threaded view onto either vertices, samples, or primitives, whereas the mesh-shading pipeline uses a cooperative thread-group.

==> tabs/buffer_teaser.tex <==
\footnotesize
\begin{tblr}[b]{
    colspec={l lr c c c c c c c c c c},
    colsep=2pt
}%
\toprule
\multicolumn{3}{l}{\textbf{Primitive Id}}                                  & $0$       &  $1$      & $2$       & $3$       & $4$       & $5$       & $6$       & $7$       & $8$       & $9$       \\
\midrule
%\multicolumn{3}{l}{\textbf{Basic Index Buffer}}     & $0,1,2$ & $2,1,3$ & $2,3,4$ & $2,4,5$ & $2,5,0$ & $0,5,6$ & $0,6,7$ & $0,7,8$ & $0,8,1$ & $1,8,9$ \\
\multirow{3}{*}{\textbf{Basic Index Buffer}}    & & & $0$ & $2$ & $2$ & $2$ & $2$ & $0$ & $0$ & $0$ & $0$ & $1$ \\
                                                & & & $1$ & $1$ & $3$ & $4$ & $5$ & $5$ & $6$ & $7$ & $8$ & $8$ \\
                                                & & & $2$ & $3$ & $4$ & $5$ & $0$ & $6$ & $7$ & $8$ & $1$ & $9$ \\
\hline
\multirow{2}{*}{\textbf{GTS}}       & \multicolumn{2}{l}{\textbf{L/R-Flag}}         &         & R        & L        & L        & L        & R        & L        & L        & L        & R        \\
                           & \multicolumn{2}{l}\textbf{{Index Buffer}}     &         & $3$       & $4$       & $5$       & 0       & $6$       & $7$       & 8       & $1$       & 9       \\
\hline
\multirow{2}{*}{\textbf{GTS Reuse}}     & \multicolumn{2}{l}{\textbf{L/R-Flag}}         &         & R        & L        & L        & L        & R        & L        & L        & L        & R        \\
                           & \multicolumn{2}{l}{\textbf{Inc Flag}}         &         & $1$       & $1$       & $1$       & 0       & $1$       & $1$       & $1$       & 0       & $1$       \\
                           %& \multicolumn{2}{l}{\textbf{Inc Prefix Sum}}   &         & $1$       & $2$       & $3$       & $3$       & $4$       & $5$       & $6$       & $6$       & $7$       \\
                           %& \multicolumn{2}{l}{\textbf{Reuse Table}}               &          &           &           &           & 0         &           &           &        & 1       &         \\ 
\bottomrule
\end{tblr}

